Language Models for Image Captioning: The Quirks and What Works

Two recent approaches have achieved state-of-the-art results in image captioning. The first uses a pipelined process where a set of candidate words is generated by a convolutional neural network (CNN) trained on images, and then a maximum entropy (ME) language model is used to arrange these words into a coherent sentence. The second uses the penultimate activation layer of the CNN as input to a recurrent neural network (RNN) that then generates the caption sequence. In this paper, we compare the merits of these different language modeling approaches for the first time by using the same state-of-the-art CNN as input. We examine issues in the different approaches, including linguistic irregularities, caption repetition, and data set overlap. By combining key aspects of the ME and RNN methods, we achieve a new record performance over previously published results on the benchmark COCO dataset. However, the gains we see in BLEU do not translate to human judgments.

==> sec.lstm.tex <==
We now examine the effect of adding Long Short Term Memory (LSTM) to the pipeline.

We take the 500-best hypotheses from the MELM system, append the LSTM logprob, and reoptimize MERT to maximize expected BLEU.  The weights are initialized to the weights learned during MELM MERT training, with the LSTM logprob weight set to 1.0.

==> ssec.lbl.tex <==
Since continuous-space LMs frequently outperform discrete models, we investigate adding continuous-space word representations to the M-ME LM in \cite{MSRCapVisCVPR2015}.
Specifically, we use the log-bilinear (LBL) features as defined in the LBL LM \cite{Mnih2007}.
In this case, the feature vector ${\bf q}_{{\bf h}, \mathcal{D}}$ is a concatenation of binary indicator vectors and LBL feature vectors.
The LBL feature vectors are defined as $\sum_{i=1}^{N-1} {\bf C}_i {\bf s}_{w_i}$, where
${\bf s}_{w_i} \in \mathbb{R}^d$ is a $d$-dimensional continuous-space representation of the $i$-th word and ${\bf C}_i \in \mathbb{R}^{d \times d}$ denotes the position-dependent context weight matrix. 
For computational efficiency, the context weight matrices ${\bf C}_i$ are made diagonal as
proposed in \cite{Mnih2008}.



==> ssec.triggers.tex <==
Using the set of visual attributes from MIL detection, \newcite{MSRCapVisCVPR2015} propose a detection-conditioned ME LM (denoted as M-ME LM in this paper) conditioned on the set of ${\it remaining}$ visual attributes $\mathcal{D} \setminus \{ {\bf h} \}$,  with ${\bf q}_{ {\bf h}, \mathcal{D} }$ being a concatenation of binary indicator vectors.
However, the ME features used in \cite{MSRCapVisCVPR2015} only capture $N$-gram
context information.
In this paper, we study the use of distant bigram features, i.e., trigger
features \cite{lau1993trigger}, to capture long-distance context information.
The indicators for trigger features can be defined as activated if predicted word is $\gamma$ and is $\gamma \notin \mathcal{D} \cap {\bf h}$, and the trigger $t^{(\gamma)}_i$ for word $\gamma$ is in ${\bf h}$.
In this paper, we use word-independent trigger features as well.
%Table\,\ref{tab:trigger_feat} gives the definition of the indicators for trigger
%features used in this paper.
The trigger features, together with the ME features in \cite{MSRCapVisCVPR2015},
form the binary feature vector ${\bf q}_{ {\bf h}, \mathcal{D} }$.
We define two kinds of triggers, i.e., left-to-right triggers and dependency
triggers.

{\bf Left-to-right trigger}: 
For each word $w$ occurred in the training data, any word $t$ occurred before
$w$ is defined as a trigger of $w$.
The top 15 frequent closed class words are removed from the set of triggers.
In this way, we can obtain a set of (trigger, word) pairs.

{\bf Dependency trigger}:
Beyond left-to-right word frequencies, we experiment with ways to infuse our model
with linguistic information grounded in a syntactic tree.  
We focus on dependency parsing, which captures pairwise dependencies between a syntactic {\it parent} and its {\it children} in the sentence.  
We use the Stanford dependency parser \cite{deMarneffe06} on the training captions, and convert each 
caption's unlabeled dependency parse to trigger features by ordering the parent and child following
the linear sentence order.  In this representation, the first word (whether parent or child) becomes the trigger for the second.

